Modeling offensive content detection for TikTok

The advent of social media transformed interpersonal communication and information consumption processes. This digital landscape accommodates user intentions, also resulting in an increase of offensive language and harmful behavior. Concurrently, social media platforms collect vast datasets comprising user-generated content and behavioral information. These datasets are instrumental for platforms deploying machine learning and data-driven strategies, facilitating customer insights and countermeasures against social manipulation mechanisms like disinformation and offensive content. Nevertheless, the availability of such datasets, along with the application of various machine learning techniques, to researchers and practitioners, for specific social media platforms regarding particular events, is limited. In particular for TikTok, which offers unique tools for personalized content creation and sharing, the existing body of knowledge would benefit from having diverse comprehensive datasets and associated data analytics solutions on offensive content. While efforts from social media platforms, research, and practitioner communities are seen on this behalf, such content continues to proliferate. This translates to an essential need to make datasets publicly available and build corresponding intelligent solutions. On this behalf, this research undertakes the collection and analysis of TikTok data containing offensive content, building a series of machine learning and deep learning models for offensive content detection. This is done aiming at answering the following research question: "How to develop a series of computational models to detect offensive content on TikTok?". To this end, a Data Science methodological approach is considered, 120.423 TikTok comments are collected, and on a balanced, binary classification approach, F1 score performance results of 0.863 is obtained.

==> sections/04data-analysis.tex <==
%!TEX root = ../CLINtemplate.tex

\section{Data analysis}\label{section:data-analysis}
For performing analyses on the dataset, different preprocessing needed to be carried out depending on the type of analysis. The following sections describe in more detail the different preprocessing steps that were taken to compile these charts. As every analysis aims to measure a different aspect or feature of the dataset, not all steps were necessarily applied to each analysis.

\subsection{Stop words}
A sentence often contains words that do not add any additional meaning to that particular sentence. These words can be removed without altering the intended message of said sentence. In NLP, these words are often removed to reduce the noise in a document, in order to achieve a more accurate or targeted analysis. Examples of English stop words  are ``a'', ``and'', ``the'', ``all'', ``do'', ``so'', ``an'', etc.~\cite{9074166,anandarajan2019text,kaur2018systematic,sarica2021stopwords}.

To this end, an existing collection of stop words, made available via the Natural Language Toolkit (NLTK) module \cite{khan2020social,sarica2021stopwords}, was used. To accommodate for the linguistic variations that are often present in social media posts, including ours, some extra words were added to this list that were specifically featured in the dataset~\cite{gouws2011contextual}:
\begin{multicols}{3}
\begin{itemize}
	\item u
	\item ur
	\item cause
	\item gonna
	\item im
	\item gon
	\item cant
\end{itemize}
\end{multicols}

Shorthand, such as ``u'' referring to the pronoun ``you'', or ``ur'' for ``you're'', among others, were added to this list. The remaining words were found to add value to the final outcome within the context of this study and therefore not removed. Words such as ``know'' are considered of value because they are most often used when referencing someone's level of intelligence in the dataset (e.g. ``Do y'all not know how to read graphs?'' or ``Lol you don't even know what the phrase means so you fall back to childish responses.'').

\subsection{Lemmatization}

Words can often be reduced to their lemma, their base or dictionary form (e.g. ``write'' is the lemma of the word ``writing''). Lemmatization allows grouping together different forms of a particular word, enabling one to analyze all of its occurrences as a single entity, thus reducing the number of variations of a particular word, which in turn improves the accuracy of the analyses~\cite{khyani2021interpretation,anandarajan2019text}. Lemmatization was chosen over stemming (which allows to reduce words with the same stem to their common form), as it achieves better accuracy [~\cite{balakrishnan2014stemming}. Lemmatization was done using the WordNetLemmatizer\footnote{\url{https://nltk.org/_modules/nltk/stem/wordnet.html}}, which is available through the NLKT module.

\subsection{Punctuation}\label{section:punctuation}

Removing special characters and punctuation markers (e.g. !, {\#}, {\$}, {\%}, {\*}, {@}) can be important for certain analyses, as these might not add extra meaning or value. An example is when using a model such as BERT, since it would remove contextual information, or for sentiment analysis, given they generally do not affect sentiment. 
It is, however, important to recognize that users on social media often use (textual) emojis to convey emotions. Removing them may therefore affect the output of the analysis~\cite{8282676,katz2022gen}.

This research therefore used a set of regular expressions to remove the punctuation and special characters.

\subsubsection{Word clouds}\label{section:wordclouds}

Word clouds are a powerful and straightforward way to visually represent a set of documents. This technique allows to quickly identify which terms are most frequently used by individuals when insulting others, or just generally when using offensive language~\cite{HeimerlFlorian2014}. 
This visualization method was applied to the offensive comments corpus and generated two word clouds. 

To this end, Figure~\ref{fig:wordcloud} provides an overview of individual words which are most used in the corpus of operandi. One can observe that the words ``People'', ``One'', ``Know'' bear the greatest weight in the chart. From this chart, it is possible to deduce that most of the offensive comments use the word ``people'', which could refer to intercultural or political discussions. Other words that seem to be important based on this chart are insults such as ``racist'', ``dumbass'', or words such as ``shut''. 

% To further explore how these individual words are actually used, the following sentences were observed in the dataset:
%% Gideon: rewritten for more conciseness/clarity

The following sentences that were observed in the dataset, illustrate how these individual words were actually used:

\begin{itemize}[itemsep=0.5ex]
	\item ``I'm not a Republican dumbass''
	\item ``shut up karen i'll kneel to the american flag burning periodt''
	\item ``They only teach you what they want you to know idiot thats why so many politicians are corrupt you gave yourself lies to fill empty space in your head''
\end{itemize}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
        \includegraphics[scale=0.20]{figures/wordcloud.png}
		\caption{based on the dataset label as offensive}\label{fig:wordcloud}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[scale=0.20]{figures/wordcloud_bigrams.png}
		  \caption{bi-grams based on the dataset label as offensive}\label{fig:wordcloud-bigrams}
     \end{subfigure}
        \caption{Word clouds}
        \label{fig:word-clouds}
\end{figure}

In addition to individual words, one can also identify the most commonly used pairs by creating a word cloud using bi-grams, such as depicted in Figure~\ref{fig:wordcloud-bigrams}. This overview shows the pairs ``white people'' and ``black people'', which could indicate that many documents are about ethnicity or race. 

The middle left of the cloud shows the words ``left wing'', which indicates that the dataset may contain quite a few comments about political opinions.
Other combinations such as ``year old'' and ``critical thinking'' are commonly used as a way to direct attention to someone's level of intelligence. 
\begin{itemize}[itemsep=0.5ex]
	\item ``Are you 14? You reason like a 14 year old girl''
	\item ``all the right wing ppl lack extreme critical thinking''
\end{itemize}
The word pair ``high horse'' on the other hand may refer to those who, according to the writer, think they are better or know better than others when it comes to a certain topic (e.g. ``so get off your racist high horse and do better'').
\begin{itemize}[itemsep=0.5ex]
	\item ``It was a mistake Karen maybe go back to school to get your IQ back??''
	\item ``I bet you don't even know what the BLM movement stands for. Dumb lib. It goes farther then striving for equality for black people.''
\end{itemize}

All in all, most of the pairs are easy to understand and relate to a particular context. Some, however, might not be that obvious, such as ``even know'' or ``go back''. These are not merely insults but combinations that need more context in order for them to make sense:
\begin{itemize}[itemsep=0.5ex]
	\item ``We've always had a foreign dependence on oil, and half you idiots don't even know what country imports the most oil to us''
	\item ``Maybe you need to go back to school and learn some writing skills before typing comments cannot even get a message out correctly.''
\end{itemize}

\subsection{Uni-grams, bi-grams and tri-grams}
Subsequent to the analysis in the previous sections, the following charts provide an overview of the top 20 most used words in offensive comments. For this analysis, three separate charts (uni-grams, bi-grams and tri-grams) were created, with two variations: one before removal of stop words and one after removal of stop words.

Figure~\ref{fig:top20-before-removing-stopwords} shows the top 20 words in the corpus, before removing stop words, providing insight into which pronouns and verbs are used within the corpus. For instance, the strong occurrence of ``you'', ``they'' and ``it'' indicates that an offensive message is most likely directed at something, a group of people or an individual. One can also notice the presence of the words ``is'', ``are'', ``be'', which all are conjugated forms of the verb ``to be'' indicates that offensive comments often include this particular verb when referring to one's actions. The progressive aspect of an action indicated by this verb further points in this direction. After removing stop words (Figure~\ref{fig:top20-after-removing-stopwords}) the results are similar to those shown in the word cloud depicted in Section~\ref{section:wordclouds}. Comparing the more predominant words from Figure~\ref{fig:wordcloud} to the top 20 shows a match. This is coherent with previous findings, as it is merely an alternate representation of the same, albeit partial, dataset.

The chart in Figure~\ref{fig:top20-bigrams-before-removing-stopwords} represents the top 20 bi-grams in the offensive subset. The predominant use of the pronoun ``you'' within the corpus is clearly visible and can be explained based on the analyses depicted in Figure~\ref{fig:top20-before-removing-stopwords}. One other bi-gram stands out: ``shut up''. Neither of these words occurred in the Top 20 chart in Figure~\ref{fig:top20-before-removing-stopwords} and only ``shut'' appeared in the Top 20 after removing stop words (Figure~\ref{fig:top20-after-removing-stopwords}), indicating that the two words carry no specific significance separately. Together, however, they contribute (more) significantly when it comes to offensive content.

After removing stop words and recalculating the top 20 bi-grams for the offensive dataset, quite a few word combinations can be identified which relate to racism, ethnicity and politics (e.g. ``white people'', ``black people'', ``left wing'', ``white supremacy'').
Additionally, other combinations seem directed towards the intelligence, knowledge, behavior or someone's appearance. Examples are ``sound like'', ``use brain'', ``sound dumb'' or ``look like''. The analysis of tri-grams (Figure~\ref{fig:top20-trigrams-before-removing-stopwords}) shows the same results as with bi-grams in Figure~\ref{fig:top20-bigrams-before-removing-stopwords} when it comes to the occurrence of the pronoun ``you''. Tri-grams are more unique than bi-grams, meaning that the unique occurrence of a tri-gram is more frequent than uni-- or bi-grams. \\The outcomes and findings previously discussed are further confirmed when looking at these tri-grams, making it possible to deduce that offensive comments are likely to address an individual's knowledge or behavior, or include some sort of call to action from the abusive language user (e.g. ``you dont know'', ``you have no'', ``you talking about'', ``look it up'').

Lastly, after removing stop words (Figure~\ref{fig:top20-trigrams-after-removing-stopwords}), the top three tri-grams in the offensive dataset are:
\begin{itemize}[itemsep=0.5ex]
	\item ``critical thinking skills''
	\item ``sound like idiot''
	\item ``get high horse''
\end{itemize}

\subsection{Length distribution}\label{section:document-features}

Another interesting metric to take into account for the dataset is the comment length. When observing Figures~\ref{fig:general-comment-length-distribution} and~\ref{fig:offensive-comment-length-distribution}, which depict the overall character comment length and the length of offensive comments in the corpus respectively, comments appear to be either rather short or long. 
Figure~\ref{fig:general-comment-length-distribution} shows that most of the comments have a length smaller or equal to $60$ characters. Comments shorter than $10$ characters usually show a user reacting to another comment with a single smiley or a single word, as shown by the examples below:
\begin{multicols}{3}
	\begin{itemize}
		\item ``LOL''
		\item ``brutal''
		\item ``<33''
		\item ``cap''
		\item ``poser''
		\item ``dumb''
	\end{itemize}
\end{multicols}

\begin{figure}
        \centering
		\includegraphics[scale=0.3]{figures/general/comment_length_distribution.png}
		\caption{Comment length distribution for both offensive and non-offensive comments}
		\label{fig:general-comment-length-distribution}
\end{figure}

In comparison, the comment length distribution for only the offensive documents, depicted in Figure~\ref{fig:offensive-comment-length-distribution}, shows that the length distribution is more evenly spread. Shorter messages are more common than longer ones, but the slump in the graph is not as significant as in the previous chart (Figure~\ref{fig:general-comment-length-distribution}).
In general, the data shows that offensive comments are more likely to contain longer texts.

\begin{figure}
        \centering
		\includegraphics[scale=0.3]{figures/offensive/comment_length_distribution_offensive.png}
		\caption{Comment length distribution of offensive comments}
		\label{fig:offensive-comment-length-distribution}
\end{figure}

Although short (one-word) messages are also used in offensive language (e.g. ``dumbass'', ``watermelonass'') the more evenly spread distribution indicates that offenders generally use more words to convey their message. Furthermore, when looking at the longest documents of the dataset, more than half of them are offensive comments.

\subsection{The use of emojis}
Gen-Z see themselves as creators, using content to express themselves and get noticed. One way to do so is by expressing their thoughts through emojis~\cite{seemiller2018generation}, making the case for further examination of the use of emojis in offensive language, as well as their relevance in this domain. 
Similarly to Section~\ref{section:wordclouds}, the frequency of occurrence of a certain (textual) emoji in the corpus was analyzed and plotted, resulting in the emoji cloud depicted in Figure~\ref{fig:most-freq-used-emojis-cloud}. Here it is important to recognize that a user can choose to use either emoticons (textual emojis) or emojis to express emotions. Both ways of expressing emotion were encountered during data collection, indicating the importance of taking both into account. In order to do this, all emoticons were converted to their textual emoji counterpart before aggregating the results and creating the final charts in Figure~\ref{fig:most-freq-used-emojis-cloud} and~\ref{fig:most-freq-used-offensive-emojis-cloud}.

Figure~\ref{fig:most-freq-used-emojis-cloud} shows that the ``face with tears of joy'', ``loudly crying face'', and ``skull'' emojis are among those most commonly used.
The ``face with tears of joy'' emoji is clearly the most used emoji in the dataset, as shown in the bar chart in Figure~\ref{fig:most-freq-used-emojis-barchart}. 
This shows that this emoji is not only used as a means to express emotions in comments having neutral to positive sentiments but also plays an important role in offensive contexts (Figure~\ref{fig:most-freq-used-offensive-emojis-barchart}). 

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
        \includegraphics[scale=0.25]{figures/general/emoji_cloud.png}
		\caption{offensive and non-offensive comments}
		\label{fig:most-freq-used-emojis-cloud}
     \end{subfigure}
     \hfill
        \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[scale=0.25]{figures/offensive/emoji_cloud_offensive.png}
		\caption{offensive comments}
		\label{fig:most-freq-used-offensive-emojis-cloud}
     \end{subfigure}
     \hfill
        \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[scale=0.24]{figures/most_frequently_used_emojis.png}
		 \caption{offensive and non-offensive comments}
         \label{fig:most-freq-used-emojis-barchart}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
        \includegraphics[scale=0.24]{figures/most_frequently_used_emojis_in_offensive_language.png}
		\caption{offensive comments}
		\label{fig:most-freq-used-offensive-emojis-barchart}
     \end{subfigure}
        \caption{Most frequently used emojis}
        \label{fig:most-frequently-used-emojis}
\end{figure}

Other emojis, such as the ``skull'' and ``loudly crying face'' emojis, do not really seem to fit in with the others, as they have a more negative connotation. The dataset developed, as a result of the desk research, shows both these emojis are often used by Gen-Z to express laughter; to this population, these emojis have all but a negative connotation.

The emojis commonly used in the overall corpus seem to be somewhat similar, even though an increase in the use of certain emojis, such as the ``clown'' emoji, can be noticed. This research shows that this particular emoji is often used by Gen-Z to highlight foolish behavior or, in the case of offensive language, to describe someone as being a fool:
\begin{figure}[h!]
    \vspace{-3mm}
    \begin{center}
		\includegraphics[scale=0.10]{figures/clowns.jpg}
		\label{fig:clowns}
	\end{center}
\end{figure}

The ``face with rolling eyes'' emoji, commonly used when expressing disapproval, is another seemingly more important emoji in offensive language: 
\begin{figure}[h!]
    \vspace{-3mm}
    \begin{center}
		\includegraphics[scale=0.08]{figures/rolling_eyes.jpg}
		\label{fig:rolling-eye}
	\end{center}
\end{figure}

The emoji-analysis showed some discrepancies in the dataset: the ``banana'' emoji seemed to be strongly represented in the dataset. 
Further investigation, however, indicated that this was due to only one comment in the corpus:

\begin{figure}[h!]
    \vspace{-3mm}
    \begin{center}
		\includegraphics[scale=0.06]{figures/bananas.jpg}
		\label{fig:bananas}
	\end{center}
\end{figure}
The extensive use of a certain emoji could be correlated to the need to express emotions, but given the excessiveness of this comment, it was considered to be an outlier --- leaving it in would distort the outcome of the emoji-cloud. 
Furthermore, it is important to emphasize that, for this specific dataset, \(8.80\%\) of comments were found to contain one or more emojis. Subsequently, only 7.18\% of all offensive comments and 10.42\% of non-offensive comments contained emojis.
